Effects of Parameter Norm Growth During Transformer Training: Inductive Bias from Gradient Descent

The capacity of neural networks like the widely adopted transformer is known to be very high. Evidence is emerging that they learn successfully due to inductive bias in the training routine, typically a variant of gradient descent (GD). To better understand this bias, we study the tendency for transformer parameters to grow in magnitude ($\ell_2$ norm) during training, and its implications for the emergent representations within self attention layers. Empirically, we document norm growth in the training of transformer language models, including T5 during its pretraining. As the parameters grow in magnitude, we prove that the network approximates a discretized network with saturated activation functions. Such "saturated" networks are known to have a reduced capacity compared to the full network family that can be described in terms of formal languages and automata. Our results suggest saturation is a new characterization of an inductive bias implicit in GD of particular interest for NLP. We leverage the emergent discrete structure in a saturated transformer to analyze the role of different attention heads, finding that some focus locally on a small number of positions, while other heads compute global averages, allowing counting. We believe understanding the interplay between these two capabilities may shed further light on the structure of computation within large transformers.

==> old_neurips/binary.tex <==
\section{Binary Cross-Entropy: Accuracy and Norm Growth} \label{sec:accuracy}

% \roy{transition can be smoother here. What have we shown so far, and what are we going to show now. In particular, why should we expect training accuracy to control the potential norm growth? this doesn't feel intuitive to me}
The $\proj$ metric reveals an interesting connection between training accuracy and norm growth for homogeneous networks.
We show that this metric is negative on a correct prediction (\autoref{thm:eq-proj}) and positive on an incorrect one (\autoref{thm:neq-proj}).
It follows that training accuracy controls the point at which the parameter norm growth reaches equilibrium, i.e., $\proj > 0$ over a batch. Thus, achieving higher accuracy allows for more norm growth. 
We first prove this for homogeneous networks with binary cross-entropy loss, and then show empirically that the relationship between accuracy and norm growth for transformer sublayers with binary cross-entropy loss is similar.

\subsection{Homogeneous Networks with Binary Cross-Entropy Loss}

We start by analyzing the case where the network is a homogeneous function $f$ followed by binary cross-entropy loss. This is similar to the case of transformers, with two important simplifications. As discussed in transformers are not strictly homogeneous, but, rather, are approximately homogeneous in the sense described in \eqref{def:approx-homo}. Second, many practical networks use the multiclass softmax cross-entropy loss instead of binary cross-entropy.
% These loss functions are quite similar from a theoretical perspective, but the binary classification version simplifies the analysis.

As discussed in \autoref{sec:norm-dynamics}, $\proj$ is useful for analyzing norm growth, assuming small learning rate. If it is negative, the weights will grow, as the gradient pushes them outwards. If it is positive, there exists some value at which the norm stops increasing, and above which, it shrinks.
Thus, the smallest norm where $\proj > 0$ acts roughly as an equilibrium point where further norm growth is bounded.

We first summarize our results informally. If the network is ``right'' in its classification, then the gradient projection is negative (and approaching zero for large $\norm{\theta}$). On the other hand, if the network is ``wrong'', the gradient projection is positive and increasing with $\norm{\theta}$. Thus, the sign of the batch-level projection depends on accuracy. If training accuracy is 100\%, then the projection will be negative throughout training, and the norm will continue to grow. If accuracy is below 100\%, then at some point the gradient projection will cross zero, causing norm growth to reach equilibrium. This means that each accuracy level has a specific norm up to which the parameters will grow.

Let $f(x; \theta)$ be a $k$-homogeneous network, and $L$ the binary cross-entropy loss. Write $f$ as shorthand for $f(x; \theta)$.
Define the prediction $\hat y = 1$ if $f > 0$ and $0$ otherwise. Assume $f \neq 0$.

\begin{theorem} \label{thm:eq-proj}
For an example $(x, y)$, if $\hat y = y$, then $\proj \leq \frac{-k \abs{f} }{\exp(\Theta(\abs{f}))} < 0$.
\end{theorem}

\begin{proof}
\begin{align}
    \proj
        &= \theta^\top \cdot \pdv{L}{f} \pdv{f}{\theta} \\
        &=  \big( \sigma(f) - y \big) \cdot \theta^\top \cdot \pdv{f}{\theta}.
\end{align}
If $f$ is $k$-homogeneous, then $\theta^\top \cdot \pdv{f}{\theta} = kf$ (proved in \autoref{thm:homo-grad}). Let $\sgn(\cdot)$ be the sign function.
\begin{align}
    \proj
    &= \big( \sigma(f) - y \big) \cdot kf \\
    % & f(k\cdot) = kf(\cdot) = kf \\
    &= \big( \sigma(f) - y \big) \cdot k \sgn(f) \abs{f} \\
    &= - \big( y - \sigma(f) \big) \cdot k \sgn(f) \abs{f} .
\end{align}
Since $\hat y = y$, the difference $y - \sigma(f)$ is asymptotically tightly bounded by a vanishing exponential in $\abs{f}$. The sign of the difference is $\sgn(f)$. Thus,
\begin{align}
    \proj
    &\leq - \frac{\sgn(f)}{\exp(\Theta(\abs{f}))} \cdot k \sgn(f) \abs{f} \\
    &= - \frac{k \abs{f}}{\exp(\Theta(\abs{f}))} ,
\end{align}
\noindent which is always less than $0$ for $\abs{f} > 0$.
\end{proof}

\begin{theorem} \label{thm:neq-proj}
For an example $(x, y)$, if $\hat y \neq y$, then $\proj \geq \frac{k \abs{f}}{2} > 0$.
\end{theorem}

\begin{proof}
We consider two cases depending on the sign of $f$.

\paragraph{Case 1} $f > 0$. Then $\hat y = 1$. Since $\hat y \neq y$,  $y=0$.
\begin{align}
    \proj
        &= \big( \sigma(f) - y \big) \cdot kf \\
        &= \big( p - 0 \big) \cdot kf
\end{align}
\noindent for some $p$ such that $\frac{1}{2} < p < 1$.
% \roy{do you really need the range for $p$? all it matters is that $p$ is positive}
Thus,
\begin{align}
    \proj
        &\geq \frac{1}{2} k \abs{f} \\
        &> 0.
\end{align}

\paragraph{Case 2} $f < 0$. Then $\hat y = 0$. Since $\hat y \neq y$,  $y=1$.
\begin{align}
    \proj
        &= \big( \sigma(f) - y \big) \cdot kf \\
        &= \big( \sigma(f) - y \big) \cdot -k\abs{f} \\
        &= \big( y - \sigma(f) \big) \cdot k\abs{f} \\
        &= \big( 1 - p \big) \cdot k\abs{f}
\end{align}
\noindent for some $p$ such that $0 < p < \frac{1}{2}$. Thus,
\begin{align}
    \proj
        &\geq (1 - \frac{1}{2}) \cdot k \abs{f} \\
        &\geq \frac{1}{2} k \abs{f} \\
        &> 0.
\end{align}

\end{proof}

Note that, as $f$ is homogeneous in $\theta$, $\abs{f}$ is monotonically increasing with $\norm{\theta}$. In any batch, the loss used to train the network is a sum of several training instances. Thus, the gradient projection $\proj$ is also the sum of the ``right'' negative term and a ``wrong'' positive term, weighted by accuracy. If accuracy is 100\%, then it will reduce to the negative quantity in \autoref{thm:eq-proj}, guaranteeing continued norm growth. However, if any instances are misclassified, then the two terms both receive nonzero weight. Since the positive term asymptotically dominates the negative one, norm growth will cease after enough time. Thus, each specific accuracy level has a value up to which norm will grow, and increasing the training accuracy increases this threshold.

% In the case where the underlying network is approximately homogeneous, rather than strictly homogeneous, these results will simply be off at most by a term that is exponentially small in $\norm{\theta}$.\roy{this requires a proof} Thus, we should expect a similar relationship between accuracy and norm growth in that case as well.

\subsection{Transformer Sublayers}

For networks with homogeneous logits and binary cross-entropy loss, we have shown that achieving higher levels of training accuracy increases the level to which the norm can grow.
We now test experimentally whether the predicted relationship holds for transformer sublayers, which we argue in \autoref{sec:transformers} are almost homogeneous, with softmax cross-entropy loss. To do this, we run experiments with randomly initialized transformer components, controlling accuracy by randomly constructing labels. For simplicity, we fix the hidden size of each component to $10$.

\paragraph{Gradient projection curves} First, we visualize the gradient projection curve as a function of norm, at different fixed accuracy levels. We do this for each component of the transformer in isolation.
% with a fixed hidden size of $10$.\roy{does this mean you use a toy transformer? with how many layers? trained on which task? Update after reading below: now I remember this part. I think we should say upfront what we are doing: trying to simulate a desired level of accuracy without actually training the network. the hidden size 10 detail doesn't belong here, you should first discuss the high level thing you are doing (which is far from trivial and might confuse many readers), and maybe later mention this.}
The transformer sublayers (discussed further in \autoref{sec:transformers}) are:

\begin{itemize}
    \item \textbf{Self attention sublayer} --- we test variants with and without biases.
    \item \textbf{Fully connected sublayer} --- we consider three variants: standard, one with biases removed, and one without biases and residual connections.
\end{itemize}

The reason we consider these variants is that, as discussed in \autoref{sec:transformers}, we assume biases and residual connections are removed in our formal analysis of the approximate homogeneity of transformers. However, both here and in \autoref{sec:transformers}, we find that transformer components behave similarly with and without these simplifying assumptions.

% Given a full network or component, 
Given a transformer sublayer,
we define the loss by first applying a random affine layer, followed by the softmax cross-entropy loss function. We randomly initialize the parameters, and vary the ``scale'' $c \geq 1$ as the independent variable. We pick a fixed accuracy level $a \in [0, 1]$. Importantly, we never train the network, computing gradients only for $\projz$. For each $c$, we do the following:
\begin{enumerate}
    \item Scale the network parameters by $c$, i.e., $\theta_0 \mapsto c\theta_0$. 
    \item For each $x$, compute $h = f(x; c\theta_0)$.
    \item We set fake labels $y$. For $a$ percent of samples, set $y=\arg \max h$. For $(1-a)$ percent, set $y$ to a value besides $\arg \max h$.
    \item Compute and record the dependent variable $\projz$ using auto-differentiation.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=.48\textwidth]{images/grad-proj/100.pdf}
    \includegraphics[width=.48\textwidth]{images/grad-proj/80.pdf}
    \newline
    \includegraphics[width=.48\textwidth]{images/grad-proj/full.pdf}
    \caption{Gradient projection with accuracy fixed at 100\% (\textbf{left}) and 80\% (\textbf{right}). The \textbf{bottom} shows norm achieving projection equilibrium as a function of accuracy. All plots share a legend.}
    \label{fig:grad-proj-components}
\end{figure}

Let $\rho_0$ be the norm of the randomly initialized parameters.
\autoref{fig:grad-proj-components} shows $\projz$ as a function of $c\rho_0$ at two fixed accuracy levels: 100\% and 80\%. With fixed 100\% accuracy, the projection is always negative and approaches 0. With 80\% accuracy, however, the projection becomes positive at a very small norm value, and it increases roughly linearly. Thus, the empirical results for transformer sublayers match the theory for homogeneous networks with binary cross-entropy loss.

\paragraph{Norm equilibrium by accuracy} We now extend this experiment to plot the norm equilibrium point for a component $f$ as a function of accuracy. To do this, we construct a random dataset of inputs $x$. We then pick various ``scales'' for the parameters $c$ and accuracy levels $a$. For the pair of independent variables $(c, a)$, we use the same method as the previous experiment to compute a sequence of $\projz$ for each $a$.
For each $a$, we then compute the first scale $c^*(a)$ in the time series at which $\projz > 0$. This corresponds to a specific norm $\rho^*(a) = c^*(a) \norm{\theta_0}$. We plot $\rho^*(a)$ as a function of $a$ in the bottom plot of \autoref{fig:grad-proj-components}.

% \begin{figure}
%     \centering
%     \includegraphics[width=.48\textwidth]{images/norm-by-acc.png}
%     \caption{Norm achieving $\proj > 0$ by accuracy for transformer sublayers.}
%     \label{fig:norm-by-acc}
% \end{figure}

\autoref{fig:grad-proj-components} shows that the equilibrium point for $\projz$ increases with accuracy, as was predicted in the theoretical analysis of homogeneous networks. The norm equilibrium point remains finite for any accuracy $<$ 100\%, going to infinity for a model that perfectly predicts the training data.

While the theoretical relationship between accuracy and norm holds empirically for transformer sublayers, for full transformers, the effect of variables like depth and width is unclear. Preliminary experiments suggest, for larger networks, the projection may remain ${\sim}0$ even for low accuracies.
% suggesting the dynamics may resemble those of a scale-invariant network \citep{li2019exponential}.
While \autoref{sec:pretrained} confirms that the norm continuously grows during pretraining of T5, we leave further analysis of full transformers to future work.

\subsection{Vanishing Step Size}

\autoref{thm:eq-proj} implies that, if 100\% accuracy is achieved, gradient flow diverges to a saturated network. But, even under these conditions, do GD and related optimizers really approach infinite norm? In this section, we show that the step size towards the saturated network vanishes, causing the norm to converge.
While this is not particularly surprising, it suggests we should expect GD to reach ``semi-saturated'' networks, rather than getting arbitrarily close to a saturated network. This resembles the empirical findings of semi-saturation in LSTMs reported by \citet{shibata2020lstm}.

\begin{theorem} \label{thm:vanishing}
Let $f: \mathbb{R}^n \rightarrow \mathbb{R}$ be a $k$-homogeneous network followed by binary cross-entropy loss.
For all $\theta$ on the $n$-sphere, assume $\norm{\nabla f_{|\theta}}$ is bounded.
Let $\rho_t = \norm{\theta_t}$.
On example $(x, y)$, if $\hat y = y$,
\begin{equation}
    \norm{\nabla L_{|\theta_t}} \leq \frac{\bigO(\rho_t^{k-1})}{\exp(\Omega(\rho_t))} .
\end{equation}
\end{theorem}

\begin{proof}
Reparameterize $\theta_t = \rho_t \hat \theta_t$, where $\hat \theta_t$ is the normalized parameter vector.

\begin{equation}
    \nabla L_{|\theta_t} = \big( \sigma(f) - y \big) \nabla f_{|\theta_t}
\end{equation}

The derivative of a $k$-homogeneous function is $(k-1)$-homogeneous, so $\nabla f_{|\theta_t} = \rho_t^{k-1} \nabla f_{|\hat \theta_t}$. Therefore,
\begin{align}
    \nabla L_{|\theta_t} 
        &\leq \frac{\nabla L_{|\theta_t}}{\exp(\Omega(\rho_t))} \\
        &=\frac{\rho_t^{k-1}}{\exp(\Omega(\rho_t))} \nabla f_{|\hat \theta_t} .
\end{align}

Finally, $\norm{\nabla f_{|\hat \theta_t}}$ lies on the $n$-sphere, so it is upper bounded by some constant by assumption:
\begin{align}
    \norm{\nabla L_{|\theta_t}}
        &\leq \frac{\rho_t^{k-1}}{\exp(\Omega(\rho_t))} \norm{\nabla f_{|\hat \theta_t}} \\
        &\leq \frac{\bigO(\rho_t^{k-1})}{\exp(\Omega(\rho_t))} .
\end{align}

\end{proof}

\autoref{thm:vanishing} suggests 
% that the parameter norm will not diverge even for a model with 100\% accuracy. The network
the gradient points along a divergent trajectory, but the step size vanishes, leading the distance travelled along the path to converge. However, there still exists a saturated network with $0$ loss at the end of the path. While the network found by training is only partially saturated,
% there is some saturated network (at the end of the trajectory) with lower loss, implying
the existence of this lower-loss saturated network suggests 
that the saturated capacity might still indirectly bound the solutions found by GD for binary cross-entropy.

% \vivekr{Maybe comment this out}
% We note that we can prevent the step size from vanishing by modifying GD to \textit{normalize} the step vector:
% \begin{equation}
%     \theta_{t+1} = \theta_t - \eta \frac{\nabla L_{|\theta_t}}{\norm{\nabla L_{|\theta_t}}} .
% \end{equation}
% As the step points in the same direction as standard GD, \autoref{thm:eq-proj} still applies for this new optimizer. So, as long as it still achieves 100\% accuracy, the parameter norm of a homogeneous network with binary cross-entropy loss diverges to infinity.\roy{again, why are we showing this? why is this optimizer interesting?}

==> old_neurips/causes_icml.tex <==
\section{Cause of Norm Growth} \label{sec:norm-dynamics}

This section discusses \emph{why} the dynamics of training should cause the parameter magnitudes to grow over the course of training.
Our analysis focuses on models simpler than transformers, but as we discuss below, we believe it sheds light on their empirical norm growth observed in \autoref{sec:norm-growth}.

% , which was the first assumption in \autoref{thm:saturation-main}.
We assume the training process produces a sequence of updates $\{\delta_t\}_{t=1}^T$ with each $\delta_t \in \mathbb{R}^n$. The parameters are updated according to $\theta_{t+1} = \theta_t + \delta_t$ .
%How does the norm change from $\theta_t$ to $\theta_{t+1}$?
Following \citet[Appendix C]{li2019exponential}, 
we expand the norm at time $t+1$ as
\begin{align}
    \norm{\theta_{t+1}}^2
        &= \norm{\theta_t + \delta_t}^2 \\
        % &= (\theta_t + \delta_t) \cdot (\theta_t + \delta_t) \\
        &= \norm{\theta_t}^2 + \norm{\delta_t}^2 + 2 \theta_t^\top \cdot \delta_t . \label{eq:norm-decompos}
\end{align}
To simplify notation, assume $\theta_0 = 0$. Unrolling the recurrence up to time $t+1$, we get
\begin{align}
    \norm{\theta_{t+1}}^2
        % &= \sum_{i=1}^t \left(\norm{\delta_i}^2 + 2\theta_i^\top \cdot \delta_i\right) \\
        &= \sum_{i=1}^t \norm{\delta_i}^2 + 2\sum_{i=1}^t \theta_i^\top \cdot \delta_i \label{eq:two-terms} .
\end{align}

\paragraph{Random walk}
To build intuition, we start with a simple case where the step vectors $\delta_t \sim \mathcal N(0, \sigma^2)$. This assumption is not realistic: the gradients at time $t+1$ depend on the gradients at time $t$, and in fact we expect the magnitude of the steps to shrink over time. Still, this case is a useful baseline for establishing expectations of how the trajectory should behave.
Let $\expval{\cdot}$ brackets denote expected value. Note that $\expval{\theta_t^\top \cdot \delta_t} = 0$. Following \eqref{eq:two-terms}, each parameter group of the network evolves as a random walk in $\mathbb{R}^n$, with the following expected norm:
\begin{equation}
    \expval{\norm{\theta_{t+1}}}
        % = \expval{\sum_{i=1}^t \norm{\delta_i}^2} + \expval{2\sum_{i=1}^t \theta_i^\top \cdot \delta_i}
        = \expval{\sqrt{\sum_{i=1}^t \norm{\delta_i}^2}}
        = \sigma \sqrt{t} = \Theta(\sqrt{t}) . \label{eq:random-walk}
\end{equation}
In other words, we expect the parameter norm to grow monotonically in time proportional to $\sqrt{t}$, diverging as $t \to \infty$.
% The growth rate is on the same asymptotic scale across each parameter. Thus, \autoref{thm:saturation-main} implies we should closely approximate a saturated network with enough time.

\paragraph{Scale-invariant networks} We now turn to a more realistic case, reflecting some simple networks, but not the transformer.\footnote{A transformer encoder is not scale-invariant, but approximately homogeneous, as proved in Appendix C.} Let $g(x; \theta_t)$ be a scale-invariant neural network, and $f(x; \theta_t)$ be the logits produced by passing $g$ through a frozen classification layer, followed by softmax cross-entropy loss $L$. Assuming standard GD (i.e.,  $\delta_t = -\eta \nabla_{\theta_t} L$), \citet{li2019exponential} show that $\theta_t^\top \cdot \delta_t = 0$, which implies
\begin{equation}
    \norm{\theta_{t+1}}^2 = \sum_{i=1}^t \norm{\delta_i}^2 .
\end{equation}
This growth pattern is monotonic, resembling the expected trend for a random walk. Assuming the training loss does not reach $0$, $\norm{\delta_t}$ will approach some nonzero asymptote, and the norm growth will be asympototically $\Theta(\sqrt{t})$.

\paragraph{Homogeneous networks} Appendix D shows that transformers are not scale-invariant, but approximately homogeneous. We will therefore analyze the setting of homogeneous networks as a proxy for transformers. An important caveat is that transformers do not necessarily well approximate homogeneous functions at initialization, but, rather, rapidly converge to do so as their norm grows. Still, we believe the simplified setting reveals insights about transformer training dynamics.

It follows from \eqref{eq:two-terms} that norm growth is controlled by $\norm{\delta_t}$, the size of each step, alongside $\theta_t^\top \cdot \delta_t$, which can be interpreted as a term augmenting random walk-like dynamics. We can diagnose whether the norm is growing according to the quantity $\drho \triangleq \norm{\delta_t}^2 + 2 \theta_t^\top \cdot \delta_t $.
Informally, $\drho$ can be thought of as a discrete-time derivative for $\norm{\theta_t}^2$. Its sign tells us whether $\norm{\theta_t}$ is increasing or decreasing.
% Recall that $\norm{\theta_t}^2$ is monotonic in $\norm{\theta_t}$.
% \roy{I am not sure why are we saying this. Also, all that follows in this paragraph is fairly trivial. Do we need to say it explicitly?} \nascomment{agree that the rest of this paragraph feels a bit distracting here} If $\drho > 0$, then $\norm{\theta_{t+1}}$ will increase after step $t$. Similarly, if $\drho < 0$, then $\norm{\theta_{t+1}}$ will decrease. Finally, if $\drho = 0$, then the norm will stay unchanged. The same facts apply over intervals: if $\drho$ is positive for all $t \in [t_i, t_j]$, then we can conclude that the norm is monotonically increasing.

Now, let $f(x; \theta_t)$ be $2$-homogeneous. We write $f(\theta_t)$ to mean the mean of $f(x; \theta_t)$ across $x$.
$f$ can be taken to reflect a transformer encoder followed by a classification layer, shown in Appendix C to be approximately homogeneous.
We derive conditions for norm growth in this setting. Importantly, the conditions depend on learning rate $\eta$ and accuracy $\alpha \in [0, 1]$, defined as the empirical expectation that the network's $\arg \max$ prediction matches the labeled class. \autoref{thm:2homo-dynamics} suggests that large learning rates and low training accuracies facilitate norm growth. Intuitively, larger $\eta$ allows the $\norm{\delta_t}^2$ term to dominate $\drho$, and, at lower $\alpha$, loss gradients will be large.

\begin{theorem} \label{thm:2homo-dynamics}
Assume standard GD for a $2$-homogeneous network $f$ with cross-entropy loss $L$. If
\begin{equation}
    \eta (1 - \alpha)^2 \min_i \norm{\nabla_{\theta_t} f_i}^2 > 16 \max_j \abs{ f_j(\theta_t) } , \label{eq:conditions}
\end{equation}
then $\norm{\theta_t}$ is increasing at time $t$, i.e. $\drho > 0$.
\end{theorem}
The proof is in Appendix B.
\autoref{thm:2homo-dynamics} identifies \eqref{eq:conditions} as a condition under which $\norm{\theta_t}$ will grow for a $2$-homogeneous network. If \eqref{eq:conditions} holds, as long as the step magnitudes converge to some nonzero value, we can conclude that $\norm{\theta_t} = \Omega(\sqrt{t})$. Breaking apart the condition in \eqref{eq:conditions}, $\norm{\nabla_{\theta_t} f_i}^2$ and $\abs{ f_j(\theta_t) }$ are both $2$-homogeneous. Thus, let us imagine their ratio stays on roughly the same order of magnitude over training. This identifies the learning rate $\eta$ and training accuracy $\alpha$ as two important factors controlling whether the norm grows.\footnote{Interestingly, if $k > 2$ for $f$, the left side will actually have a greater homogeneity coefficient than the right side. 
As our focus is $2$-homogeneous transformers, we do not explore this further, but believe there may be interesting implications for higher homogeneity networks, e.g. cascades of ReLU layers.}
% \footnote{\autoref{thm:2homo-dynamics} assumes homogeneity: a property met approximately by a variety of neural architectures, not just transformers. Thus, we hope these results advance the general understanding of neural network training dynamics.}

\paragraph{Language modeling} Notably, practical language models cannot be expected to come close to 100\% accuracy without severely overfitting the pretraining data.\footnote{In natural language, the same prefix could ambiguously correspond to two different next tokens, implying that 100\% accuracy on the training set is not even possible.}
Thus, in the context of transformer language modeling, it makes sense to imagine $\alpha$ remains low over the course of training. If the theory translates to approximately homogeneous transformers, it thus predicts that norm growth should be largely modulated by the learning rate, with a critical threshold $\eta^*$ above which the norm will grow over training.
% \roy{related to the comment above: we have so far not restricted ourselves to LM transformers, but discussed transformers in general. what about non-LM transformers?} \nascomment{probably advisable to keep broad scope in most places, and relegate all LM/application specific claims/notes to one place (e.g., this labeled paragraph).  if we keep mentioning LM everywhere throughout the paper, reviewers might think the paper is too niche}

\paragraph{Weight decay}
%\subsection{Weight Decay}
Weight decay regularizes the loss by the squared $\ell_2$ norm, modulated by a decay factor $\lambda$. For GD, a weight decay optimizer can be written as
\begin{equation}
    \delta_t = -\eta \nabla_{\theta_t} L -  \lambda \theta_t . \label{eq:wd}
\end{equation}
Intuitively, the new term $ \lambda \theta_t$ will influence each step to point towards $0$.
Whereas we expect large learning rates to be associated with norm growth, large weight decay should hinder it. 
% Potentially, if $\lambda$ is large enough, it may be the case $\drho < 0$.
% \will{Might be worth mentioning that $\nabla_{\theta_t}$ is $2$-homogeneous, whereas $\theta$ is $1$-homogeneous. This means that weight decay becomes negligible as the norm gets bigger, and all that really matters is it doesn't dominate at the start of training.}\roy{seems relevant, yes}
% \will{I potentially have some more theory to put here}
While we leave developing a more complete theoretical story to future work, 
here we empirically investigate the interplay of learning rate $\eta$ and weight decay $\lambda$ by training a variety of transformer language models on Wikitext-2 for $1$ epoch.\footnote{$1$ epoch is chosen because of the computational cost of running this experiment over a large grid. In \autoref{sec:norm-growth}, we found that growth continued beyond $1$ epoch using the default AdamW settings.} We use the AdamW \citep{DBLP:journals/corr/abs-1711-05101} optimizer, varying $\lambda$ and $\eta$ across a range of common values, keeping all other hyperparameters constant.
\autoref{fig:norm-grids} visualizes the phase transition for norm growth as a function of $\lambda, \eta$.
% For SGD, we observe positive norm growth for $\eta$ roughly less than $1$e${-}3$ and $\lambda$ roughly less than $1$e${-}5$. For AdamW, 
The norm growth behavior seems to largely depend on weight decay, with a threshold for $\lambda$ lying between $0.01$ and $0.001$. While the trend likely depends on the optimizer, we can infer for AdamW at least that norm growth is probable when $\lambda = 0.01$, which is a common choice, e.g., reflecting default settings in PyTorch.
As the network architecture is fixed across all runs, the effect of hyperparameters like the depth and width is unclear.

\begin{figure}[t]
    \centering
    % \includegraphics[width=\columnwidth]{images/grid/SGD.pdf}
    \includegraphics[width=\columnwidth]{images/grid/AdamW-encoder.pdf}
    \caption{Norm growth over the first epoch, varying $\eta, \lambda$. The triangle shows the default AdamW hyperparameters in PyTorch.}
    \label{fig:norm-grids}
\end{figure}


% \paragraph{Vanishing steps} For models with 100\% accuracy, arbitrary saturation cannot be achieved because the step size eventually vanishes.
% % In this case, there is still a loss-decreasing trajectory diverging from the point at which training gets stuck, implying some saturated network effectively bounds the loss of the network found by training.
% In some sense, vanishing step size is an artifact of designing optimizers to find local minima, rather than divergent trajectories towards infinite-norm networks.
% Existing optimizers could be modified to remove this vanishing effect, for example, by normalizing the gradient vector.
% We leave open the question of how making these changes---and thus reaching more saturated networks---affects the performance of practical neural networks.
% Although---at least in the case of our transformer language modeling experiments---making such changes are not necessary to reach full saturation. \nascomment{never leave open questions in the appendix.  I suggest you move this discussion back up in to section 3, where you discussion the less-than-100\% accuracy assumption}

\paragraph{Limitations}
Our analysis is limited in several ways as a model for norm growth in transformers. First, as mentioned, \autoref{thm:2homo-dynamics} assumes full homogeneity whereas transformers are approximately homogeneous. Second, it assumes standard GD, whereas a variety of more complicated optimizers are used to train transformer language models in practice. Finally, as mentioned above, weight decay might counteract growing norm.
Importantly, our empirical results (\autoref{sec:norm-growth}) hint that in practice these limitations do not prevent transformer parameter norm from growing.


==> old_neurips/diff_eq.tex <==
\textbf{EVERYTHING AFTER THIS IS INCOMPREHENSIBLE}

\section{One Layer}

Let $f_w(x) = w \cdot x$ and the binary cross-entropy loss 
\begin{equation}
    L(w) = E_{x,y} \big[ -\big( y \log \sigma(f_w(x)) + (1 - y) \log (1 - \sigma(f_w(x))) \big) \big] .
\end{equation}

% Similar to https://deepnotes.io/softmax-crossentropy#derivative-of-cross-entropy-loss-with-softmax, we have $\pdv{L}{f} = p - y$

Note the following: 
\begin{equation}
    \sigma'(x) = \sigma(x) \big(1 - \sigma(x) \big) = \frac{e^{-x}}{(e^{-x} + 1)^2}
\end{equation}

We start by assuming gradient flow, i.e. that the parameters follow the gradient over time.

\begin{align}
    \dv{w}{t} &= -\pdv{L}{w} \\
              &= -\pdv{L}{f} \pdv{f}{w}\\
              &= E_{x,y} \big( y - \sigma(w\cdot x) \big) x
\end{align}

Assuming $x$ is Gaussian with mean $0$, then $E_x w \cdot x = 0$. Thus $\pdv{L}{w} \cdot w = 0$, which implies divergence, by the Arora paper argument. What happens with two layers?

\section{Two Layers}

Instead, let $f_{U,w}(x) = w \cdot \relu(Ux)$. Let $h = Ux$. By the analysis in the last section, we have:

\begin{equation}
    \dv{w}{t} = E_{x,y} \big( y - \sigma(w\cdot h) \big) h
\end{equation}

Now, using the chain rule, we also compute the derivative for $U$:

\begin{align}
    \dv{U}{t} &= -\pdv{L}{U} \\
              &= -\pdv{L}{f}\pdv{f}{h}\pdv{h}{Ux}\pdv{Ux}{U} \\
              &= E_{x,y} \big( y - \sigma(w\cdot x) \big) w \cdot \mathbbm{1}_{>0}(Ux) \cdot x
\end{align}

\paragraph{Start of old norm analysis}

Before continuing, let's check whether the orthogonality property holds for large $w$.

\begin{align}
    \pdv{\norm{w}}{w} &= \pdv{}{w} \sqrt{\sum{w_i^2}} \\
                      &= \frac{1}{2} \big( \sum{w_i^2} \big)^{-1/2} \cdot 2w \\
                      &= \frac{w}{\norm{w}}
\end{align}
 
 Now we put them together using chain rule (using $w(t)$ to be explicit about our varying parameter):
 
 \begin{align}
     \dv{\norm{w(t)}}{t} &= \pdv{\norm{w(t)}}{w} \cdot \dv{w(t)}{t}\\
                      &= \frac{w(t)}{\norm{w(t)}} \cdot \big( y - \sigma(w(t)\cdot x) \big) x \\
                      &= \frac{w(t)}{\norm{w(t)}} \cdot \big( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \big) x
 \end{align}
 
 Can we solve $\dv{\norm{w}}{t} = \frac{wx}{\norm{w}}$? That would be illumating. Let's take the expectation over $x$ from unit ball. Under this assumption, we have that $w \cdot x = 0$. Thus, the derivative is $0$.


\section{ODEs to solve}

We need to solve either

\begin{equation}
    \dv{\norm{w(t)}}{t} = \frac{w(t)}{\norm{w(t)}} \cdot \left( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \right) x
\end{equation}

or 

\begin{equation}
    \dv{w(t)}{t} = \left( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \right) x
\end{equation}

\begin{align}
    \dv{w(t)}{t} &= \left( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \right) x\\
    \equiv dw(t) &= \left( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \right) x dt\\
    \int_0^t dw(t) &= \int_0^t \left( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \right) x dt\\
    w(t) &=  t y x - \int_0^t \frac{xe^{w(t)x}}{e^{w(t)x} + 1} dt\\
    &= tyx - \log \left(1 + e^{w(t) x}\right)
\end{align}

where $x\in\mathbb{R}^n$ is our constant input, $y\in\{0, 1\}$ is our constant target, and $w(t)\in\mathbb{R}^n$ is our learned linear form. $u = 1 + e^{w(t)x}$ so $u' = xe^{w(t)x}$. Therefore $x\sigma(w(t) x) = \frac{u'}{u} \Rightarrow \int \frac{1}{u} du = \log u = \log 1 + e^{w(t) x}$


Ok Will's claim:

\begin{equation}
    \int \frac{e^{w(t)x}}{e^{w(t)x} + 1} dw(t) = \frac{1}{x} \log(1 + e^{w(t)x})
\end{equation}

\begin{equation}
    \int ... dw_1(t) dw_2(t) dw_3(t)... = 
\end{equation}


Proof. Just take the derivative.

\begin{align}
    \dv{}{w(t)} \frac{1}{x} \log(1 + e^{w(t)x^T}) & = \frac{1}{x} \frac{1}{1+e^{w(t)x^T}} e^{w(t)x^T} \cdot x\\ 
    &= \frac{e^{w(t)x^T}}{1+e^{w(t)x^T}} .
\end{align}

$\dv{}{w(t)} = [\pdv{}{w_i(t)}]$

\section{Our Formalization of Martin's Thoughts}

By chain rule, $\dv{w(t)}{t} = x f'(t)$. We have an expression for the left side, let's plug that in.

\begin{align}
    \left( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \right) x &= f'(t) x \\
    \left( y - \frac{e^{f(t)x^2}}{e^{f(t)x^2} + 1} \right) &= f'(t)
\end{align}

Now we assume $y = 1$. We have $1 - \sigma(f(t)x^2) = f'(t)$.

We have something like $f'(t) = 1 - \sigma(f(t))$, up to constants. We integrate using separation of variables:

\begin{align}
    f'(t) &= 1 - \sigma(f(t)) \\
    \frac{df}{1 - \sigma(f(t))} &= dt \\
    \int \frac{df}{1 - \sigma(f(t))} &= \int dt \\
    f(t) + e^{f(t)} &= t .
\end{align}

$f(t)$ has to be getting large to satisfy $f(t) + \exp(f(t)) = t$. And if $f(t)$ is getting large, then we know this equation just approaches $\exp(f(t)) = t$, which implies $f(t) = \log t$.

It also works out similarly in the other case, i.e. with $y=0$.

What happens with expected value? Seems like it might not work. Also, this argument won't generalize to a two-layer network.

Define $\Delta = w(t) \cdot \nabla_{w(t)} L$. Simplifying and substituting, we have $\Delta = w(t)\cdot \dv{w(t)}{t}$. We can compute time derivative of this value as
\begin{align}
    \dv{\Delta}{t} &= \dv{}{t} w(t)\cdot \dv{w(t)}{t}\\
    &= \dv{w(t)}{t}\cdot \dv{w(t)}{t} + w(t)\cdot \dv[2]{w(t)}{t}
\end{align}


\begin{equation}
    d \norm{w}^2 = \norm{dw}^2 + 2 w^T dw
\end{equation}

where $dw = \pdv{w}{t} dt$


\begin{align}
    \dv {w(t)}{t} &= \left( y - \frac{e^{w(t)x}}{e^{w(t)x} + 1} \right) x\\
    \Delta(t) &= w(t) \dv{w(t)}{t}
\end{align}

Parameters of the plot are $\rho$ and $\Delta$. Let $\mathcal U_\rho$ be a uniform distribution over the ball of radius $\rho$. We want to plot the following following vector as a function of $\Delta, \rho$:

\begin{equation}
\myexpval_{w \sim \mathcal U} \langle \dv{\Delta}{t}, \dv{\norm{w}}{t} \rangle
\end{equation}

If $U$ is \textit{any} network with radius $\rho$, don't expect any feedback loop. But what about if $U$ is constrained to solutions that actually separate the data? In this case, we expect a feedback loop.

Note: we are "collecting" the values of delta.

\section{Will's numerical hessian example}

\begin{align}
    \theta = (\theta_1, \theta_2) \\
    L = 2\theta_1 + \theta_2^2 \\
    \pdv{L}{\theta} = (2, 2 \theta_2) \\
    \dv{\theta}{t} = -(2, 2 \theta_2) \\
    \pdv[2]{L}{\theta} = ((0, 0), (0, 2)) \\
    \dv[2]{w}{t} = \dv{}{t} \pdv{L}{\theta} = (0, -2 \dv{\theta_2}{t}) = (0, 4\theta_2) 
\end{align}


Let $f(\theta) = \theta\cdot \nabla_\theta L$. Then using a first-order Taylor expansion, we have that

\begin{align}
    f(\theta + \Delta\theta) &= f(\theta) + \Delta\theta \cdot \nabla_\theta f(\theta)\\
    &= f(\theta) + \Delta\theta\cdot \nabla_\theta\left(\theta\cdot \nabla_\theta L(\theta)\right).
\end{align}

Expanding the partial derivative in (89), we get

\begin{align}
    \nabla_\theta\left(\theta\cdot \nabla_\theta L(\theta)\right) &= \left[\pdv{}{\theta_i} \sum_{j}\theta_j\cdot \pdv{L}{\theta_j}\right]_i\\
    &= \left[\pdv{}{\theta_i} \theta_i\cdot \pdv{L}{\theta_i}\right]_i\\
    &= \left[\pdv{L}{\theta_i} + \theta_i\pdv[2]{L}{\theta_i}\right]_i\\
    &= \nabla_\theta L + \theta\odot \mathrm{diag} \textbf {J}(\nabla_\theta L) 
\end{align}

Just as a sanity check, $f : \mathbb{R}^n \to \mathbb{R}$, so we expect $\nabla_\theta f$ to have dimensionality $n\times 1$.

 Define our update $\Delta\theta = -\alpha\nabla_\theta L$. We want to take the directional derivative as follows

\begin{align}
    \lim_{\alpha\to 0} \frac{f(\theta - \alpha\nabla_\theta L) - f(\theta)}{\alpha} &= \frac{f(\theta) + \Delta\theta\cdot \nabla_\theta\left(\theta\cdot \nabla_\theta L(\theta)\right) - f(\theta)}{\alpha}\\
    &= \frac{-\alpha\nabla_\theta L^T (\nabla_\theta L  + \theta\odot \mathrm{diag} \textbf {J}(\nabla_\theta L))}{\alpha}\\
    &= -\nabla_\theta L^T (\nabla_\theta L  + \theta\odot \mathrm{diag} \textbf {J}(\nabla_\theta L))
\end{align}

Further, $\dv{\norm{\theta}}{t} = -\frac{\theta}{\norm{\theta}}\cdot \nabla_\theta L$. Expanding, we get

\begin{align}
    -\frac{\theta}{\norm{\theta}}\cdot \nabla_\theta L &= \norm{\nabla_\theta L} \cos{\phi}
\end{align}

Where $\phi$ is the angle between $\theta$ and $-\nabla_\theta L$. 

Computing $\mathrm{diag}~\textbf {J}(\nabla_\theta L))$ directly is still difficult! So we have to use the Hutchinson trace estimator, which says that $Tr(A) = \mathbb{E}[z^TAz]$ and $z_i\sim \text {Rademacher} (1/2)$. The trace, however, is a scalar. So we need some manipulation to get it to work with (101). First note that in the proof for the Hutchinson estimator, they rely on the key fact that
\begin{equation}
    \mathbb{E}[zz^T] = \Sigma + mm^T,
\end{equation}

where $\Sigma$ is the covariance matrix of $z$. If $\Sigma = I$, then we retrieve our generic estimator. However, what if $\Sigma = \theta I$. Then we get
\begin{align}
    \text{Tr} (A (\theta I)) &= \text{Tr} (A\mathbb{E}[zz^T])\\
    &= \mathbb{E} [\text{Tr} (A zz^T)] \\
    &= \mathbb{E} [z^T A z].
\end{align}

Further, we know that
\begin{equation}
    \text{Tr} (A (\theta I)) = \theta^T \textbf{diag } A
\end{equation}

Now we just need to get (100) in the form we want,

\begin{align}
    \nabla_\theta L^T (\nabla_\theta L  + \theta^T\odot \mathrm{diag} \textbf {J}(\nabla_\theta L)) &= \nabla_\theta L^T \nabla_\theta L + \nabla_\theta L^T (\theta\odot \mathrm{diag} \textbf { J}(\nabla_\theta L))\\
    &= \nabla_\theta L^T \nabla_\theta L + \mathbb{E} [z^T \textbf { J}(\nabla_\theta L)) z]
\end{align}

Where the covariance of $z$ is $\text{diag }\nabla_\theta L\odot \theta$ and its mean is 0. Notice that now we're just iterating Hessian vector products $\textbf {J}(\nabla_\theta L)) z$ (or vector Hessian products $z^T \textbf {J}(\nabla_\theta L))$, whichever is faster).

==> old_neurips/impact.tex <==
\section*{Broader Impact}

Our contributions are foundational in focus, and thus it is hard to precisely predict their social impact. However, it is important to understand the inductive bias of neural models in order to truly explain their decisions. Thus, we hope our efforts contribute to the large project that is the interpretability of neural systems \citep{lipton2016mythos}.

% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

==> old_neurips/intro_icml.tex <==
\section{Introduction} \label{sec:intro}

Modern neural networks achieve good generalization performance across many different tasks and application domains. In order for these highly overparameterized models to generalize well, there ought to be some implicit inductive bias or capacity control in the learning algorithms, but it is an interesting open question what this is, or even how to characterize it.
In particular, transformers \citep{vaswani2017attention} like BERT \citep{devlin2019bert}, XLNet \citep{yang2019xlnet}, RoBERTa \citep{liu2019roberta}, and T5 \citep{raffel2019t5} have pushed the state of the art on an impressive array of NLP tasks.
% Each of these highly overparameterized models is ``pretrained'' on an unsupervised objective resembling language modeling.
% , and then the representation from the pretrained model is ``fine-tuned'' to solve a supervised downstream task.
Because these models are so large, their success is tied to the question of how capacity is restricted by training. What prevents them from overfitting,\roy{well, for once, they train on enormous amounts of data and never reach close to 0 train loss?} allowing pretrained representation to generalize well to other problems?
\will{I realize now that this framing may be what caused the ICML meta-reviewer to expect claims about generalization. Is there some way to change it?}

% \nascomment{if you make the change I propose above, explain a bit more what these things are:  norm growth, GD (spell out), saturated networks (once you do this you can trim the explanations in the new section 2) ... also add the new section to the road map.}
In this work, we take the perspective that thoroughly understanding the dynamics of gradient descent (GD) might clarify the biases or capacity restrictions imposed by training for transformers.
We start by making a somewhat surprising empirical observation (\autoref{sec:norm-growth}): the parameter $\ell_2$ norm grows proportional to $\sqrt{t}$ during the training of T5 \citep{raffel2019t5} and other transformers.\roy{what about the possible explanation by  one of the ICML reviewers about the connection between the LR scheduler and $\sqrt{t}$?}
We continue by studying the causes of this trend, relying on established theory about the learning dynamics of homogeneous networks.
We show theoretically that the parameter norm in homogeneous networks grows with training, identifying learning rate, training set accuracy, and weight decay as factors modulating this trend (\autoref{sec:norm-dynamics}). Though transformers are only \textit{approximately} homogeneous, these results partly explain our empirical observations.
%In a simplified formal 

We then consider the effect of norm growth on network behavior (\autoref{sec:effect}).
We prove that, with some light assumptions, any network where the parameter norm diverges during training approaches a \emph{saturated} network \citep{merrill2020aformal}: a restricted network variant whose discretized representations are understandable in terms of formal languages and automata.
% Theoretically, transformers increasingly approximate saturated networks as their norm grows.
Empirically, we find that internal representations of pretrained transformers resemble their saturated counterparts, whereas for randomly initialized transformers, they do not. This suggests that the norm growth implicit in training guides transformers to approximate saturated networks, justifying analyzing saturated networks \citep{merrill2019sequential} as a means to explore the inductive biases of NLP architectures, and the structure of their representations. We show, both theoretically and empirically, how saturation can be leveraged to identify two different types of attention heads within a transformer: one which attends locally to a small number of positions, and one which attends uniformly over the full sequence, enabling counting.

Combined, our theoretical and empirical results shed light on the inductive biases built into the transformer architecture when trained with GD algorithms, and could serve as a tool to analyze it, visualize it, and improve its performance.

\section{Background and Related Work} \label{sec:related-work}

\subsection{Deep Learning Theory}

A simple case where deep learning theory has studied the generalization properties of GD is matrix factorization \citep{gunasekar2017implicit, arora2019implicit, razin2020implicit}. It has been observed that deep matrix factorization leads to low-rank matrix solutions. \citet{razin2020implicit} argued theoretically that this bias of GD cannot be explained as an implicit regularizer minimizing some norm. Rather, they construct cases where all parameter norms diverge during GD.

% In order to explain the inductive bias of training feedforward networks, recent work has analyzed the dynamics of training from a new perspective.
Similar ideas have emerged in recent works studying feedforward networks.
Analyzing biasless ReLU networks with cross-entropy loss, \citet{poggio2019theoretical, poggio2020complexity} show that the \textit{magnitude} ($\ell_2$ norm) of the parameter vector continues to increase during GD, whereas its \textit{direction} converges. \citet{li2019exponential} present a similar argument for any network that is \emph{scale-invariant}, meaning that scaling the parameters by a constant does not change the output. This property leads the norm to monotonically increase during training.
Studying \emph{homogeneous} networks, \citet{telgarsky2020directional} show that the gradients become \emph{aligned} as $t \to \infty$, meaning that their direction converges to pointing away from the origin. This means the norm will grow monotonically with $t$.
The perspective developed by these works challenges the once conventional wisdom that the parameters converge to a local minimum during GD training. Rather, it suggests that GD follows a norm-increasing \textit{trajectory} along which network behavior stabilizes.
% However, such work makes simplifying assumption about feedforward networks--such as removing biases--and does not directly extend to more complicated networks like transformers.
These analyses motivate investigation of this trajectory-driven perspective of training.

From a statistical perspective, work in this vein has considered the implications of these training dynamics for margin maximization \citep{poggio2019theoretical, nacson2019lexicographic, lyu2019gradient}. While these works vary in the networks they consider and their assumptions, they reach similar conclusions: GD follows trajectories diverging in the direction of a max-margin solution. As margin maximization produces a simple decision boundary, this property suggests better generalization than an arbitrary solution with low training loss. This point of view partially explains why growing norm is associated with better generalization performance.

\will{Should we also cite the claim in the backpropaganda paper that low norm is actually not better, i.e., conventional understanding of weight decay is flawed?}

\subsection{Formal Language Theory}

% But
Norm growth has another interpretation for NLP models. Past work characterizes the capacity of networks with infinitely scaled norm in terms of formal language and automata theory.
\citet{merrill2019sequential} and \citet{merrill2020aformal} propose \emph{saturation}, a framework for theoretical analysis of the capacity of NLP architectures. A network is analyzed by assuming it \emph{saturates} its nonlinearities, which means replacing functions like $\sigma$ and $\tanh$ with step functions. Formally, this is equivalent to uniformly scaling the weights by a constant approaching $\infty$, which allows us to define saturated networks as follows:
\begin{definition}[Saturation; \citealp{merrill2020aformal}] \label{def:saturation}
Let $f(x; \theta)$ be a neural network with inputs $x$ and weights $\theta$.
The \textit{saturated network} $\sat f(x; \theta)$ is defined\footnote{Where the limit is taken pointwise.}
\begin{equation*}
    \sat f(x; \theta) = \lim_{c \rightarrow \infty} f(x; c\theta) .
\end{equation*}
\end{definition}
Saturation reduces complex connectionist NLP models to discrete computational models resembling automata or circuits, making some kinds of theoretical analysis easier. For many common architectures, the saturated capacity is known to be significantly weaker than the full capacity of the network with rational-valued weights \citep{merrill2019sequential}, which, classically, is Turing-complete for even simple RNNs \citep{siegelmann1992turing}.
% \footnote{Geometrically, the saturated capacity corresponds to a set of limit points in parameter space.}

For example, one can hand-construct an RNN or LSTM encoding a stack in its recurrent memory \citep{kirov2012fractals}.
Stacks are useful for processing compositional structure in linguistic data \citep{chomsky1956three}, e.g. for semantic parsing.
However, a saturated LSTM does not have enough memory to simulate a stack \citep{merrill2019sequential}. Rather, saturated LSTMs resemble classical counter machines \citep{merrill2019sequential}: automata limited in their ability to model hierarchical structure \citep{merrill2020linguistic}.
Experiments suggest that LSTMs trained on synthetic tasks learn counter-like representations \citep{weiss2018, suzgun2019lstm}, and that they fail on tasks requiring stacks and other deeper models of structure \citep{suzgun2019memory}.
Similarly, \citet{shibata2020lstm} found that LSTM language models trained on natural language data acquire saturated representations approximating counters.

Recent work extends saturation analysis to transformers \citep{Hahn_2020, merrill2019sequential, merrill2020aformal}. The saturated transformer reduces to an ``arg max'' hard attention machine where attention focuses on the values with maximum key-query similarity. In this case of ties, attention is distributed uniformly over all values with maximal similarity. While the capacity of this machine is not fully understood, it can implement a counting mechanism similar to the LSTM. \citet{bhattamishra2020ability} show that transformers can learn counting tasks using this construction, and that they struggle on tasks requiring more complicated structural representations.
\citet{ebrahimi-etal-2020-self} find that attention patterns of certain heads can emulate bounded stacks, but that this ability falls off sharply for longer sequences.
Thus, experiments suggest that the synthetic tasks LSTMs or transformers can learn are predicted by their saturated counterparts. \citet{merrill2020aformal} conjecture that the saturated capacity might represent a class of behaviors implicitly learnable by GD, although it is unclear \emph{a priori} why this should be the case. This work will argue that saturation arises in transformers due to the norm growth in SGD training dynamics.


==> old_neurips/lstm.tex <==
\section{LSTMs}

Whereas we argued both theoretically and empirically that the transformer is approximately $1$-homogeneous, we now show that the LSTM--even without biases--is not approximately homogeneous. This represents a formal difference between the two architectures.

First, we define the LSTM architecture.

\begin{definition}
Let $x_1, \cdots, x_t \in \mathbb{R}^n$ be a sequence of input vectors. An LSTM is a parameterized function that produces two output sequences: the cell state $c_1, \cdots, c_t \in \mathbb{R}^m$ and output state $h_1, \cdots, h_t \in \mathbb{R}^m$. Define the computation recurrently according to:
\begin{align}
    f_t &= \sigma(W^fx_t + U^fh_{t-1}) \label{eq:lstm-f} \\
    i_t  &= \sigma(W^ix_t + U^ih_{t-1}) \label{eq:lstm-i} \\
    o_t  &= \sigma(W^ox_t + U^oh_{t-1}) \label{eq:lstm-o} \\
    \tilde c_t &= \tanh(W^cx_t + U^ch_{t-1}) \label{eq:lstm-c} \\
    c_t &= f_t c_{t-1} + i_t \tilde c_t \\
    h_t &= o_t \tanh(c_t) .
\end{align}
\end{definition}

Note that, as we did for the transformer, we omit bias terms.

\begin{lemma}
There do not exist $k_c, k_h : \mathbb{N} \rightarrow \mathbb{N}$ such that, for all $t$, $c_t$ is approximately $k_c(t)$-homogeneous, and $h_t$ is approximately $k_h(t)$-homogeneous.
\end{lemma}

\begin{proof}
Assume by way of contradiction that such constants $k_c(t), k_h(t)$ exist. Then the input to $\sigma$ in \eqref{eq:lstm-f}, \eqref{eq:lstm-i}, and \eqref{eq:lstm-o} is the sum of two homogeneous terms, so it is monotonically increasing. Thus, by \autoref{thm:sigmoid-error}, $f_t$, $i_t$, and $o_t$ are approximately $0$-homogeneous. The same argument applies for \eqref{eq:lstm-c} with $\tanh$ instead of $\sigma$, showing that $\tilde c_t$ is approximately $0$-homogeneous as well.

The rest of the proof focuses on the equation $c_t = f_t c_{t-1} + i_t \tilde c_t$. We have assumed that, for all $t$ $c_t$ is approximately $k_c(t)$-homogeneous for all $t$. Since the approximate homogeneity of the terms must be equal if $c_t$ is approximately homogeneous
\end{proof}

\will{TODO: Argument here not complete, finish or remove}


==> old_neurips/multiclass.tex <==
\section{Softmax Cross-Entropy} \label{sec:softmax}

We now shift to a similar empirical setting with a multiclass loss function. We randomly initialize a full transformer, and interpret the output of the transformer as logits for a softmax cross-entropy loss function.
We find that the theory about projections developed for binary cross-entropy loss in \autoref{sec:accuracy} does not hold for the more commonly used softmax cross-entropy loss. Our empirical results suggest that the bounding effect of accuracy on the gradient projection equilibrium point goes away. At random initialization (\autoref{fig:proj-by-classes}), the gradient projection is marginally positive. However, we also find that the number of classes is inversely proportional to the gradient projection. This means that with many classes, the projection will be very close to zero, and the norm will grow $\bigO(\sqrt{t})$ like for a scale invariant network \citep[cf.][]{arora2018theoretical}. Note that we plot the cosine similarity of the projection, rather than the unnormalized dot product, in order to enable comparison between networks with different numbers of parameters. Further, in \autoref{fig:proj-by-scale}, we find that the cosine similarity quickly goes to $0$ as the parameters are scaled up from their standard initialization by a scalar $c$.

\will{What happens if the step size vanishes? Do we want another plot that explores that possibility?}

\will{Should we add in a random linear layer to be more standard?}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/scale-softmax/proj-1.pdf}
    \caption{Normalized gradient projection for randomly initialized transformers. The projection is marginally positive, but goes to $0$ as the number of classes increases. The error bars are over several random initializations of the same architecture.}
    \label{fig:proj-by-classes}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/scale-softmax/proj-scales.pdf}
    \caption{Gradient projection for randomly initialized transformers as the weights are multiplied by a scalar $c$. The projection vanishes rapidly to $0$ as $c$ increases. The projection is normalized to a cosine distance to enable comparison between models of different sizes.}
    \label{fig:proj-by-scale}
\end{figure}

==> old_neurips/norm_sgd.tex <==
\section{Normalized SGD}

Finally, we propose a simple new optimization method, which we call normalized SGD (NormSGD). The method is exactly equivalent to standard SGD, except that the gradient vector is renormalized at every step to a fixed, constant magnitude. For small enough step size, the trajectory with NormSGD approximates the trajectory of standard SGD, except that never gets ``stuck'' at flat regions. Thus, this type of optimization method would not make sense if our goal was to converge to some local minimum--however, given the trajectory perspective of training, it should achieve similar results to standard SGD.

We train a single model on FashionMNIST with both standard SGD and NormSGD,\roy{we mostly talked about transformers so far, so it is surprising to see a vision experiment here. worth saying something about this} comparing the performance and norm growth. In [Figure X], we find that the models perform comparably. As expected, the norm increases more for NormSGD than for standard SGD. We also train the same model where the labels are manipulated so that the network has 100\% accuracy at initialization. In this case, we [hopefully] find that the norm does not converge.

Combined with our formal analysis of norm growth, we take these results as evidence that reaching a local minimum is not necessary for achieving good performance. Rather, following a trajectory of increasing norm is sufficient for converging in performance. We can also view the trajectory found by NormSGD as an estimate of the trajectory standard SGD would continue along if the step size did not vanish. From this point of view, since the NormSGD model with fixed 100\% accuracy does not appear to converge in norm, it appears there is a loss-decreasing trajectory from the point reached by standard SGD to some infinite-norm network. Thus, we can view the saturated capacity as bounding the capacity of the network reached by SGD, i.e. there exists some saturated network with lower loss than the network found by SGD.

==> old_neurips/old_why.tex <==
\section{Why does the Norm Grow?}

\subsection{Random Walk}

Before looking at actual SGD, we consider the simpler case where the step is a random walk. This is perhaps a reasonable model of the dynamics at the beginning of training, where the gradients are quite random.

Let $\theta \in \mathbb{R}^n$. Let's assume each step has magnitude $\delta$ and direction chosen uniformly from the $n$-sphere. This means, for any $n>1$, there is some angle $\alpha$ uniform between $0$ and $\pi$ between our step and the orthogonal $n-1$-hyperplane. We express the parameter update recurrently in $\alpha$:

\begin{align}
    \norm{\theta_{t+1}}^2 &= \norm{0 + \delta \cos \alpha}^2 + \norm{\theta_t + \delta \sin \alpha}^2 \\
    &= \delta^2 \cos^2 \alpha + \norm{\theta_t}^2 + 2 \norm{\theta_t} \delta \sin \alpha + \delta^2 \sin^2 \alpha \\
    &= \delta^2 + \norm{\theta_t}^2 + 2 \norm{\theta_t} \delta \sin \alpha
\end{align}

Taking the expectation over $\alpha$, the third term vanishes:

\begin{equation}
    \myexpval_\alpha \norm{\theta_{t+1}}^2 = \delta^2 + \norm{\theta_t}^2
\end{equation}

Assume $\theta_0 = 0$. Taking the sum over all $i \leq t$, we get

\begin{align}
    \myexpval_{\alpha_1, \dots, \alpha_t} \norm{\theta_t}^2 &= t\delta^2 \\
    \implies \myexpval_{\alpha_1, \dots, \alpha_t} \norm{\theta_t} &= \delta \sqrt{t}
\end{align}

So, with a random walk, we see that the norm is expected to grow $\sim \sqrt{t}$. Intuitively, we expect this to be an upper bound on the growth with SGD, since with SGD, the step size will probably decrease over time.

\subsection{Feedback Loop}

But, importantly, common practical neural network architectures are not scale invariant.\roy{Is this your observation? Li and Arora's?} So why should the norm still diverge during their training?\roy{did you show somewhere that their norm grows? I am not sure I understand the ``why'' here} We believe\roy{believe? ``show'' maybe?} there is a feedback loop where norm growth leads to the network to become exponentially closer to scale invariant, and increased scale invariance leads to norm growth. Let's make this more precise.

\will{Should we define this here? or only when we're talking about specific networks?}

\paragraph{Scale invariance leads to norm growth} Following Li and Arora, we express the change in the squared norm $\Delta \norm{\theta_t}^2$ at time $t$ as

\begin{equation}
    \Delta \norm{\theta_t}^2 = \norm{\Delta \theta_t}^2 + 2 \theta_t^\top \cdot \Delta \theta_t
\end{equation}

Assuming $\theta_0 = 0$ (approximately true), we get the following by summing over both sides

\begin{align} \label{eq:two-series}
    \norm{\theta_t}^2 = \sum_{i=1}^t \norm{\Delta \theta_i}^2 + 2 \cdot \sum_{i=1}^t \theta_i^\top \cdot \Delta \theta_i
\end{align}
The form in \eqref{eq:two-series} provides a lot of intuition about the norm growth dynamics. Importantly, the norm is made up of two independent series. The first series is monotonically increasing, since each term is positive (potentially diverging or converging). If the network is scale invariant, then $\theta_i^\top \cdot \Delta \theta_i = 0$ for SGD-like methods since scale invariance implies $\theta^\top \cdot \nabla_\theta L = 0$. Thus, the second series becomes negligible if the network is approximately scale invariant, and the norm is approximated well by a monotonically increasing series. \roy{Maybe add something like ``we conclude that networks that are \textbf{approximately scale-invariant exhibit norm growth}''?}

% TODO: Talk about difference between forward and backward here.

\paragraph{Norm growth leads to scale invariance} To formalize this, we study \textit{scaling error}, i.e. the difference between an activation function's output when it is input is scaled versus unscaled. We show that, for sigmoid and softmax, this error vanishes exponentially in the input norm. We start by analyzing the simpler sigmoid, and then show that the same result holds for softmax.

\begin{theorem} \label{thm:sigmoid-error}
The scaling error for $\sigma$ vanishes exponentially in the preactivation magnitude, i.e. for all $c > 1$ and $x \neq 0$,
\begin{equation}
    \abs{\sigma(cx) - \sigma(x)} \leq O(\exp(-\abs{x})) .
\end{equation}
\end{theorem}

\begin{proof}
When $x > 0$, we have
\begin{align}
    \abs{\sigma(cx) - \sigma(x)}
        &= \sigma(cx) - \sigma(x) \\
        % &= 1 - \sigma(x) \\
        &\leq 1 - \sigma(\abs{x}) \\
        &= \frac{1}{\exp(\abs{x}) + 1} \\
        &= O(\exp(-\abs{x})).
\end{align}
When $x < 0$, we have
\begin{align}
    \abs{\sigma(cx) - \sigma(x)}
        &= \sigma(x) - \sigma(cx) \\
        &\leq 1-\sigma(\abs{x}) + 0 \\
        &= O(\exp(-\abs{x})).
\end{align}
\end{proof}

\begin{theorem} \label{thm:softmax-error}
The elementwise scaling error for $\softmax$ vanishes exponentially in the preactivation norm, i.e. for all $c > 1$, $x \in \mathbb{R}^n$ s.t. $x \neq 0$, and $1 \leq i \leq n$,
\begin{equation}
    \abs{\softmax(cx)_i - \softmax(x)_i} \leq \exp(-O(\norm{x})) .
\end{equation}
\end{theorem}

\begin{proof}
The proof closely follows that of \autoref{thm:sigmoid-error}, but is more involved.
We consider two cases: $x_i = \max(x)$, and $x_i \neq \max(x)$.
% We consider three cases: $x_i = \max(x)$, $x_i = \min(x)$, and $\min(x) < x_i < \max(x)$. We assume without loss of generality that $\min(x) \neq \max(x)$, since if this is true, softmax outputs the (scale-invariant) uniform distribution.

\paragraph{Case 1} $x_i = \max(x)$.

\begin{align}
    \abs{\softmax(cx)_i - \softmax(x)_i}
    &= \softmax(cx)_i - \softmax(x)_i \\
    &\leq 1 - \softmax(x)_i \label{eq:simplified-softmax} \\
    &= 1 - \frac{\exp(x_i)}{\sum_j \exp(x_j)} \\
    &\leq 1 - \frac{\exp(\max(x))}{\exp(\max(x)) + (n-1)\exp(\min(x))} \\
    &= 1 - \frac{1}{1 + (n-1)\exp(\min(x) - \max(x) + k)} \\
    &= 1 - \sigma(\max(x) - \min(x) - k) \\
    &= 1 - \sigma(O(\norm{x})) \\
    &= \exp(-O(\norm{x})) .
\end{align}

\roy{where did $k$ come from in (24)? also, I feel like more explanations might help. E.g., in (20), I see why increasing $x_i$ by $c$ would make it's softmax value larger, but is it necessary that it will make all other values smaller (28)? maybe if I think about it a bit more I will be convinced, but it wasn't trivial to me}
\paragraph{Case 2} $x_i \neq \max(x)$.

\begin{align}
    \abs{\softmax(cx)_i - \softmax(x)_i}
    &= \softmax(x)_i - \softmax(cx)_i \\
    &\leq 1 - \max(\softmax(x)) - 0 \\
    &= 1 - \softmax(\max(x)) ,
\end{align}

\noindent which is identical to \eqref{eq:simplified-softmax}.

% \paragraph{Case 2} $x_i = \min(x)$.

% \begin{align}
%     \abs{\softmax(cx)_i - \softmax(x)_i}
%     &= \softmax(x)_i - \softmax(cx)_i \\
%     &\leq \softmax(x)_i \\
%     &= \frac{\exp(x_i)}{\sum_j \exp(x_j)} .
% \end{align}

% At this point, let $\mintwo(x)$ denote the second minimal element of $x$ (we know this exists since we assumed $\max(x) > \min(x)$).

% \begin{align}
%     &\leq \frac{\exp(\min(x))}{\exp(\min(x)) + (n-1)\exp(\mintwo(x))} \\
%     &= \frac{1}{1 + (n-1)\exp(\mintwo(x) - \min(x))} \\
%     &= \sigma(\min(x) - \mintwo(x) + k) \\
%     &= 1 - \sigma(\mintwo(x) - \min(x) - k) \\
%     &= 1 - \sigma(O(\norm{x})).
% \end{align}

\end{proof}

Finally, we prove that the composition of two such functions also has vanishing scaling error. This is a nice property because it justifies analyzing modules of a network in order to see whether the full network has vanishing scaling error.

\begin{theorem}
Let $f: \mathbb{R}^m \rightarrow \mathbb{R}$ and $g: \mathbb{R}^n \rightarrow \mathbb{R}^m$. Suppose that, for both $f$ and $g$, the scaling error is bounded by $\exp(-O(\norm{X}))$. Then the scaling error of the composition $f \circ g$ is also bounded by $\exp(-O(\norm{X}))$.
\end{theorem}

\begin{proof}
\begin{align}
    f(g(cx) ) 
        &\leq f \big( g(x) \pm \exp(-O(\norm{x})) \big) \\
        &\leq f(c'g(x)) \\
        &\leq f(g(x)) \pm \exp(-O(\norm{x})) .
\end{align}

\roy{what is $c'$? didn't get (32) and (33)}
Therefore,
\begin{equation}
    \abs{f(g(cx)) - f(g(x))}\leq \exp(-O(\norm{x})) .
\end{equation}
\end{proof}

\subsection{Homogeneity Analysis}

The implication of scaling errors vanishing is that growing the parameters leads the non-scale-invariant regions of the network to quite rapidly become scale-invariant if the preactivation norm grows with $\norm{\theta}$. We will analyze whether this growth occurs by leveraging the related property of \textit{homogeneity}.\roy{I think you need to spend a little more time explaining what is the role of this section. In particular, it wasn't clear to me what you mean by ``whether this growth occurs''}

\paragraph{Homogeneity} A function $f(x; \theta)$ is $k$-homogeneous in $\theta$ if $f(x; c\theta) = c^kf(x; \theta)$. Note that scale invariance is equivalent to $0$-homogeneity.
As argued by  Li and Arora, many components of neural networks are homogeneous for some $k$. Li and Arora (2020) show how various functions in the network transform the homogeneity, expressing the homogeneity of their output as a function of their input (in certain cases, the homogeneity of the output is undefined). Applying these facts over the full network graph, we can recursively compute the homogeneity of the full network (which is potentially undefined if the network is not homogeneous for any $k$). We relax this algorithm to allow exponentially vanishing scaling error to count as approximate $0$-homogeneity. Given \autoref{thm:sigmoid-error} and \autoref{thm:softmax-error}, we immediately have the following facts: $\sigma, \softmax : k \rightarrow 0$. This is an approximate version of the homogeneity behavior of normalization layers like layer norm without learnable parameters.\roy{I didn't understand the last sentence. Also, a roadmap of the current section would help before diving into the next paragraph}

\paragraph{Softmax cross-entropy} Now, consider a network with $L$ feedforward layers without biases where layers $1, \cdots, L-1$ have ReLU activations, and the final layer has $\softmax$ followed by cross-entropy loss. In other words:

\begin{align}
    f &= \softmax(W_L \relu(W_{L-1} \cdots \relu(W_1x))) \\
    L &= \mathrm{CE}(f, y)
\end{align}

\roy{You are assuming no bias right? better say it}

The input $x$ is $0$-homogeneous.\roy{what does it mean that the input is 0-homogeneous? homogeneity is a property of function. Are you implying that you can think of the input as the identity function?}  Each linear transformation $W_i$ increases the homogeneity by $1$\roy{why? was this shown by Li and Arora? you need to say it if so, or prove otherwise}, and $\relu$ does not affect the homogeneity\roy{same comment}. Thus, the preactivations of $f$ is $L$-homogeneous. Since softmax is approximately scale-invariant for homogenous input\roy{0-homogeneous? what is homogeneous without a number?} with high enough norm, $f$ is approximately scale invariant, which implies that loss also rapidly approaches scale invariance.\roy{I didn't understand the last claim. Are you saying that it doesn't matter that the input is $L$-homogeneous, the softmax at the end ``cancels'' it in some way? does this follow from the theorems in 2.2?}  

This example illustrates how a network with cross-entropy loss should quite rapidly become scale-invariant if their input is $k$-homogeneous for some $k$. If the norm gets sufficiently large to become scale invariant, the network should be guaranteed to diverge.\roy{the term divergence is overloaded and might confuse the readers, might be a good idea to say upfront what we mean by divergence in this paper, or make sure to discuss divergence of parameter norms rather than networks}

\section{Norm Flow}

Inspired by these results, we propose a method to visualize the interaction of norm and scale invariance for a given architecture. For each architecture, we plot a two-dimensional vector field, where one axis $\rho$ represents norm, and the other represents the scalar quantity $-\theta^\top \cdot \dv{L}{\theta}$. The vectors at each point represent the expected gradient over all $\theta$ of radius $\rho$ and inputs $x,y$.

While the quantity $-\theta^\top \cdot \dv{L}{\theta}$ is not a direct measure of scale invariance, we know that it equals $0$ when the architecture is scale invariant. Thus, if there is a feedback loop between norm growth and scale invariant, we might expect to see this reflected in the flow of the vector field.

A practical challenge here is computing the derivative $\dv{}{t} \big( -\theta^\top \cdot \dv{L}{\theta} \big)$. Assuming gradient flow, we can express this as

\begin{equation}
    \dv{}{t} \big( \theta^\top \cdot \dv{\theta}{t} \big) = \big(\dv{\theta}{t}\big)^2 + \theta^\top \cdot \dv[2]{\theta}{t} .
\end{equation}

We have access to $\theta$ and $\dv{\theta}{t}$ directly through auto-differentiation. However, computing $\dv[2]{\theta}{t}$, which roughly represents the acceleration of each parameter over time, is not as simple. In order to compute it, we derive an expression in for it in terms of $\theta$ and $\dv{\theta}{t}$:

\begin{align}
    \dv[2]{\theta}{t}
        &= \dv{}{t} \big( \dv{\theta}{t} \big) \\
        &= \pdv{}{\theta} \big( \dv{\theta}{t} \big) \dv{\theta}{t} \\
        &= \pdv{}{\theta} \big( {-}\pdv{L}{\theta} \big) \cdot -\pdv{L}{\theta} \\
        &= \pdv[2]{L}{\theta} \pdv{L}{\theta} . \label{eq:hvp}
\end{align}
 
The quantity in \eqref{eq:hvp} is a Hessian-vector product, which can be efficiently computed using auto-differentiation.
Putting it all together, we have
 
\begin{equation}
    \dv{}{t} \big( \theta^\top \cdot \dv{\theta}{t} \big) =
    \big(\pdv{L}{\theta}\big)^2 + \theta^\top \cdot \pdv[2]{L}{\theta} \pdv{L}{\theta} .
\end{equation}

\subsection{Cross-Entropy Loss}

We now analyze any network with softmax cross-entropy loss, where the logits are an approximately homogeneous function $f(x; \theta)$. By \autoref{thm:softmax-error}, the predictions $\softmax(f(x, c\theta))$ are approximately scale-invariant. However, the loss does not exhibit this same scale invariance, as the $\log$ in cross-entropy undoes the negative exponential in the error term, preventing it from vanishing. In fact, for large $c$, the loss will be infinite for any network that misclassifies at least one example, as $\lim_{x \rightarrow 0} {-}\log x = \infty$.

A key property of $f$, though, is that, while the loss and its derivatives are not scale-invariant, the \textit{direction} of the derivative is approximately scale-invariant:

\begin{align}
    \pdv{}{\theta} L(c\theta)
    &= \pdv{L}{f} \cdot \pdv{f}{\theta} \\
    &= \big( \softmax(f(c\theta)) - y \big) \cdot \nabla_\theta f(c\theta) \\
    &\approx \big( \softmax(f(c\theta)) - y \big) \cdot \nabla_\theta (c^kf(\theta)) \\
    &= c^k \cdot \big( \softmax(f(c\theta)) - y \big) \cdot \nabla_\theta f(\theta) \\
    &\approx c^k \cdot \big( \softmax(f(\theta)) - y \big) \cdot \nabla_\theta f(\theta) , \label{eq:grad}
\end{align}

\noindent whose direction does not depend on $c$.

Combining these observations gives an interesting picture of the loss landscape. There is a small region around zero norm where the landscape is mysterious. Once we leave this region by traveling outward on some ray $c\theta$, the error term vanishes, and both the predictions and gradient direction become scale-invariant. Any direction that misclassifies at least one example has very high loss and points back to zero. Thus, it acts as a ``wall'' that reflects the parameters back toward the mysterious region around zero. Eventually, the parameters exit this region along a ray that achieves zero or close-to-zero training loss, at which point they continue to grow, rather than being reflected. Thus, there is an implicit process that guides the norm to grow towards solutions with zero training loss.

Another consequence is that, once a solution separating the data correctly is achieved, loss should go to zero exponentially in norm. Thus happens because the gradient in \eqref{eq:grad} contains the factor $\softmax(f(\theta)) - y$, which, under these conditions, goes to zero exponentially in $\norm{\theta}$. Thus, the network parameters will not diverge: instead, they will move on an increasing path with vanishing step size, eventually converging to some final norm. Importantly, the reason why the norm converges is not because we have gotten stuck at a local minimum. Rather, it is because the gradient step has gotten sufficiently small.

% Finally, we prove that the composition of two approximately scale-invariant functions is also scale-invariant.

% \begin{theorem}
% Let $f: \mathbb{R}^m \rightarrow \mathbb{R}$ and $g: \mathbb{R}^n \rightarrow \mathbb{R}^m$. Suppose that, for both $f$ and $g$, the scaling error is bounded by $\exp(-O(\norm{X}))$. Then the scaling error of the composition $f \circ g$ is also bounded by $\exp(-O(\norm{X}))$.
% \end{theorem}

% \begin{proof}
% \begin{align}
%     f(g(cx) ) 
%         &\leq f \big( g(x) \pm \exp(-O(\norm{x})) \big) \\
%         &\leq f(c'g(x)) \\
%         &\leq f(g(x)) \pm \exp(-O(\norm{x})) .
% \end{align}

% \roy{what is $c'$? didn't get (32) and (33)}
% Therefore,
% \begin{equation}
%     \abs{f(g(cx)) - f(g(x))}\leq \exp(-O(\norm{x})) .
% \end{equation}
% \end{proof}

==> old_neurips/preliminaries.tex <==
\section{Formal Preliminaries} \label{sec:preliminaries}


Let $\nabla_\beta g$ be the gradient of a scalar-valued function $g$ with respect to $\beta$. We may omit $\beta$ when it is clear from context.
%We formally define saturation, which was mentioned in \autoref{sec:intro}.
 \citet[][Appendix C]{li2019exponential} discuss \textit{scale invariance}, which means that a network's output does not change when its parameters are uniformly scaled.
\begin{definition}[Scale invariance; \citealp{li2019exponential}]
A function $f(x; \theta)$ is \textit{scale-invariant} in $\theta$ if for all $c > 0$, inputs $x$, and parameters $\theta$, $f(x; c\theta) = f(x; \theta)$.
\end{definition}
\citet{li2019exponential} observe that, for any scale-invariant $f$, $\theta^\top \cdot \nabla_{\theta} f = 0$. They show how this property is related to monotonic norm growth.

Scale invariance also naturally relates to saturation. The saturated capacity of a scale-invariant network is equivalent to the full capacity, as scaling $\theta$ to $\infty$ does not change the output. \emph{Homogeneity} generalizes scale invariance:

% While scale invariance and homogeneity are useful tools for characterizing some network components, they fall short of characterizing all common network pieces. For example, the output homogeneity of softmax is, strictly speaking, undefined. To extend these tools to softmax and other network components, we
% relax the definition to \textit{approximate} scale invariance and homogeneity. Here and throughout the paper, we will make use of asymptotic $\bigO$, $\Omega$, and $\Theta$ notation.
% We define approximate scale invariance as approximate $0$-homogeneity.
% In Appendix C, we show that the homogeneity properties in \autoref{tbl:homogeneity} extend to approximate homogeneity.
% Appendix D defines the transformer architecture, and shows that it is approximately homogeneous.\footnote{We prove this without biases and residual connections. However, we find it holds empirically even without simplification. This recalls findings of \citet{lyu2019gradient} with feedforward networks.}

==> sections/other.tex <==
\section{Other Lemmas}

The following lemmas are useful for analyzing the quantity $\theta_t^\top \cdot \delta_t$ in homogeneous networks.

\begin{lemma} \label{thm:homo-grad}
For $\theta \in \mathbb{R}^n$, let $f: \mathbb{R}^n \rightarrow \mathbb{R}^m$ be a function such that $f(\theta)$ is $k$-homogeneous in $\theta$. Then,
\begin{equation}
    \jac (f) \cdot \theta = k f(\theta) .
\end{equation}
\end{lemma}

\begin{proof}
For all $c \geq 1$,
\begin{align}
    f(c\theta) &= c^k f(\theta) \\
    \dv{}{c} f(c\theta) &= \dv{}{c} c^k f(\theta) \\
    \jac_{c \theta}(f) \cdot \theta &= kc^{k-1} f(\theta) .
\end{align}
Now, let $c=1$. We get
\begin{equation}
    \jac_{\theta}(f) \cdot \theta = k f(\theta) .
\end{equation}
\end{proof}

\begin{corollary}
For $\theta \in \mathbb{R}^n$, let $f: \mathbb{R} \rightarrow \mathbb{R}^m$ be a function such that $f(\theta)$ is $k$-homogeneous in $\theta$. Then,
\begin{equation*}
    \nabla f^\top \cdot \theta = k f(\theta) .
\end{equation*}
\end{corollary}

\subsection{Bounds on Loss Gradient Norm}

Let $x,y$ represent data points.
Let $L$ be expected softmax cross-entropy loss applied to neural network logits $f(x; \theta)$.

\begin{lemma} \label{thm:grad-ub}
\begin{equation*}
    \norm{\nabla_f L}^2 \leq 2.
\end{equation*}
\end{lemma}

\begin{proof}
Recall that
\begin{equation}
    \nabla_f L = \expval{\softmax(f(x; \theta)) - y} .
\end{equation}
We can maximize the norm by making all predictions incorrect and, for each example, concentrating all of probability mass of $\softmax$ at a different index than $y$. This means:
\begin{equation}
    \norm{\nabla_f L}^2 \leq 1^2 + (-1)^2 = 2 .
\end{equation}
\end{proof}

Now, define the accuracy $\alpha$ of a network $f$ as
\begin{equation}
    \alpha = \mathrm{Pr} \big( \arg \max f(x; \theta) = \arg \max y \big) .
\end{equation}

\begin{lemma} \label{thm:grad-lb}
Let $\alpha$ be the accuracy of $f$. Then,
\begin{equation*}
    \norm{\nabla_f L}^2 \geq \frac{1}{4}(1 - \alpha)^2 .
\end{equation*}
\end{lemma}

\begin{proof}
Introduce the notation $\nabla_f L(z)$ for the loss evaluated on a specific example $z = \langle x, y \rangle$ (assuming $Z$ total examples). Let $\mathcal W$ denote the set of examples where $f$ is ``wrong'', and $\mathcal R$ denote the set where $f$ is ``right''. Then:
\begin{align}
    \norm{\nabla_f L}^2
        &= \norm{\frac{1}{Z} \sum_{z} \nabla_f L(z)}^2 \\
        &\geq \norm{ (1 - \alpha) \inf_{z \in \mathcal W} \nabla_f L(z) + \alpha \inf_{z \in \mathcal R} \nabla_f L(z) }^2 \\
        &= \norm{ (1 - \alpha) \inf_{z \in \mathcal W} \nabla_f L(z) }^2 \\
        &= (1 - \alpha)^2 \norm{ \inf_{z \in \mathcal W} \nabla_f L(z) }^2 \\
        &\geq (1 - \alpha)^2 \left( 1 - \frac{1}{2} \right)^2 \\
        &= \frac{1}{4} (1 - \alpha)^2 .
\end{align}
\end{proof}
